ArchesWeather & ArchesWeatherGen: a deterministic and generative model for efficient ML weather forecasting

Weather forecasting plays a vital role in today's society, from agriculture and logistics to predicting the output of renewable energies, and preparing for extreme weather events. Deep learning weather forecasting models trained with the next state prediction objective on ERA5 have shown great success compared to numerical global circulation models. However, for a wide range of applications, being able to provide representative samples from the distribution of possible future weather states is critical. In this paper, we propose a methodology to leverage deterministic weather models in the design of probabilistic weather models, leading to improved performance and reduced computing costs. We first introduce \textbf{ArchesWeather}, a transformer-based deterministic model that improves upon Pangu-Weather by removing overrestrictive inductive priors. We then design a probabilistic weather model called \textbf{ArchesWeatherGen} based on flow matching, a modern variant of diffusion models, that is trained to project ArchesWeather's predictions to the distribution of ERA5 weather states. ArchesWeatherGen is a true stochastic emulator of ERA5 and surpasses IFS ENS and NeuralGCM on all WeatherBench headline variables (except for NeuralGCM's geopotential). Our work also aims to democratize the use of deterministic and generative machine learning models in weather forecasting research, with academic computing resources. All models are trained at 1.5{\deg} resolution, with a training budget of $\sim$9 V100 days for ArchesWeather and $\sim$45 V100 days for ArchesWeatherGen. For inference, ArchesWeatherGen generates 15-day weather trajectories at a rate of 1 minute per ensemble member on a A100 GPU card. To make our work fully reproducible, our code and models are open source, including the complete pipeline for data preparation, training, and evaluation, at https://github.com/INRIA/geoarches .

==> figs/full_ablation_table.tex <==
\begin{table}[ht]
\label{full_ablation_tab}
  \centering
\begin{small}
\begin{sc}
\begin{tabular}{lllccccccccc}
\toprule
L & Name & Z500 & T850 & Q700 & U850 & V850 & T2m & SP & U10m & V10m \\
\midrule
2 & ArchesWeather-S w/o CLA & 55.116 & 0.722 & 0.577 & 1.432 & 1.485 & 0.594 & 69.768 & 0.942 & 0.993 \\
29 & ArchesWeather-S w/o FT & 50.632 & 0.676 & 0.554 & 1.354 & 1.402 & 0.567 & 63.447 & 0.878 & 0.922 \\
9 & ArchesWeather-S & 49.365 & 0.672 & 0.551 & 1.345 & 1.395 & 0.567 & 62.710 & 0.870 & 0.914 \\
6 & ArchesWeather-Sx4 & 47.042 & 0.652 & 0.541 & 1.299 & 1.347 & 0.549 & 59.291 & 0.838 & 0.881 \\
\midrule
10 & ArchesWeather-M w/o CLA & 51.820 & 0.688 & 0.558 & 1.393 & 1.425 & 0.572 & 65.616 & 0.888 & 0.934 \\
25 & ArchesWeather-M w/o FT & 48.720 & 0.646 & 0.541 & 1.295 & 1.340 & 0.552 & 61.572 & 0.834 & 0.877 \\
18 & ArchesWeather-M & 48.022 & 0.644 & 0.540 & 1.290 & 1.336 & 0.551 & 60.981 & 0.830 & 0.872 \\
39 & ArchesWeather-Mx4 & 43.911 & 0.616 & 0.522 & 1.230 & 1.271 & 0.528 & 55.688 & 0.789 & 0.828 \\
\midrule
23 & ArchesWeather-L w/o FT & 46.846 & 0.623 & 0.531 & 1.245 & 1.288 & 0.540 & 59.031 & 0.801 & 0.841 \\
44 & ArchesWeather-L & 46.321 & 0.621 & 0.530 & 1.242 & 1.286 & 0.540 & 58.649 & 0.798 & 0.838 \\
18 & ArchesWeather-Lx2 & 44.346 & 0.606 & 0.519 & 1.207 & 1.251 & 0.525 & 55.956 & 0.776 & 0.815 \\
\bottomrule
\end{tabular}
\end{sc}
\caption{Ablation: RMSE scores of key weather variables for variants of our model. w/o FT does not use recent data for the last 50k steps, and w/o CLA additionally does not use Cross-Level-Attention. The -Sx4, -Mx4 and -Lx2 are models ensembles using 4, 4, and 2 models respectively.}
\end{small}

\end{table}

==> figs/main_table_old.tex <==
\begin{table*}[t]
  \centering
\vskip 0.15in
\begin{small}
\begin{sc}
\begin{tabular}{lllccccccccc}
\toprule
                  & \textbf{Res.} & \textbf{Cost} & \textbf{Z500} & \textbf{T850} & \textbf{Q700} & \textbf{U850} & \textbf{V850} & \textbf{T2m} & \textbf{SP} & \textbf{U10m} & \textbf{V10m} \\
\midrule
IFS HRES              &    0.1º           &                                                                & 42.30         & 0.625         & 0.556         & 1.186         & 1.206         & 0.513        & 60.16       & 0.833        & 0.872        \\
\midrule
Pangu             & 0.25º         & 2880                                                           & 44.31         & 0.620         & 0.538         & 1.166         & 1.191         & 0.570        & 55.14       & 0.728        & 0.759        \\
GraphCast         & 0.25º         & 2688                                                           & 39.78         & 0.519         & 0.474         & 1.000         & 1.02          & 0.511        & 48.72       & 0.655        & 0.683        \\
\midrule
%Keisler GNN           & 1º            & 11                                                             & 66.87         & 0.816         & 0.658         & 1.584         & 1.626         & N/A          & N/A         & N/A          & N/A          \\
SphericalCNN      & 1.4º          & 384                                                            & 54.43         & 0.738         & 0.591         & 1.439         & 1.471         & N/A          & N/A         & N/A          & N/A          \\
Stormer           & 1.4º          & 256                                                            & 45.12         & \bfu{0.607}         & 0.527         & \bfu{1.138}         & \bfu{1.156}         & 0.570        & \bfu{53.77}       & \bfu{0.726}        & \bfu{0.760}        \\
NeuralGCM ENS (50) & 1.4º          & 7680                                                           & \bfu{43.99}         & 0.658         & 0.540         & 1.239         & 1.256         & N/A          & N/A         & N/A          & N/A          \\
\midrule
ArchesWeather-M           & 1.5º          & 11                                                            & 48.1          & 0.645         & 0.538         & 1.294         & 1.342         & 0.550        & 60.9        & 0.834        & 0.877        \\
ArchesWeather-L & 1.5º & 22 & 46.32 & 0.621 & 0.530 & 1.242 & 1.286 & 0.540 & 58.649 & 0.798 & 0.838 \\

ArchesWeather-Mx4 & 1.5º          & 44                                                           & \textbf{44.36} & \textbf{0.619} & \textbf{0.523}	&1.235	&1.277	& 0.530	& 56.3	& 0.793	& 0.832       \\
ArchesWeather-Lx2 & 1.5º & 44 & \textbf{44.35} & \bfu{0.606} & \bfu{0.519} & \textbf{1.207} & \textbf{1.251} & \bfu{0.525} & \textbf{55.956} & \textbf{0.776} & \textbf{0.815} \\
\bottomrule

\end{tabular}
\end{sc}
\end{small}
  \caption{Comparison of AI weather models on RMSE scores for key weather variables with 24h lead-time. Cost is the training computational budget in V100-days. Best scores for training resolution coarser than 1º in \bfu{underlined bold}, second best scores in \textbf{bold}.}
  \label{table:main}
\end{table*}

%48.02	0.6435	0.5399	1.2905	1.3362	0.5514	60.9819	0.8296	0.8723
